A Dynamic Model of Private Asset Allocation

We build a state-of-the-art dynamic model of private asset allocation that considers five key features of private asset markets: (1) the illiquid nature of private assets, (2) timing lags between capital commitments, capital calls, and eventual distributions, (3) time-varying business cycle conditions, (4) serial correlation in observed private asset returns, and (5) regulatory constraints on certain institutional investors' portfolio choices. We use cutting-edge machine learning methods to quantify the optimal investment policies over the life cycle of a fund. Moreover, our model offers regulators a tool for precisely quantifying the trade-offs when setting risk-based capital charges.

==> to_do_list.tex <==
\newpage
\section{To Do List. \textcolor{red}{NOT for public release!}}

Not in any particular order of importance:

\begin{enumerate}
    \item Numerical algorithm for solving the model
    \begin{itemize}
        \item The $\varrho_{P}=0$ case gets rid of $\mu_P$ as a state variable. This model can be solved using standard numerical techniques. Use this solution to guide the GP fitting for the general case by treating $\varrho_{P}$ as a quasi-state variable
    \end{itemize}
    \item General reporting of results:
    \begin{itemize}
        \item Certainty equivalent wealth (especially when doing comparative statics)
        \item What does wealth growth rates look like? Sharpe ratios? expected portfolio returns? portfolio volatility? Plot the terminal wealth distribution (especially when doing comparative statics). Condition on the business cycle.
        \item Start simulations from different initial states. For example, it need not be the case that $w_0=1$ and $k_0=0$, we can just as well start from the ``maintenance phase''
        \end{itemize}
    \item Presentation of results for the exercise where the naive LP uses a model without business cycles to navigate a world with business cycles
    \begin{itemize}
        \item Report conditional cumulative default boundaries (conditional on the initial starting state)
    \end{itemize}
    \item Section on whether or not return unsmoothing is necessary
    \begin{itemize}
        \item Do comparative statics for $\varrho_{P}$. At some point, there is sufficient serial correlation that the LP investor can take advantage despite facing implementation lags
        \item Do comparative statics for adjustments costs. At some point, the adjustment becomes easy enough for the LP to take advantage of return predictability
    \end{itemize}
    \item Model section
    \begin{itemize}
        \item Derive autocorrelation function, means, volatility, etc., for the realized PE return process. The idea is to check whether or not $\varrho_{P,1}$ and $\varrho_{P,2}$ can be separately identified by using different lags. Also check long-run returns (e.g., 2 periods, 3 periods, etc.)
    \end{itemize}
    \item Modeling of the risk budget
    \begin{itemize}
        \item Make the risk weights a function of the local volatilities? Perhaps the LP knows that serial correlation doesn't matter for actual returns, but it makes the returns look smoother on paper which can have advantages when it comes to reporting, for example, earnings.
    \end{itemize}
    \item Calibration
    \begin{itemize}
        \item Risk Budgeting: as Hui highlighted the risk budgeting constraint can have the interesting effect of constraining on local volatility and thus potentially showcasing how an investor with same risk aversion but different risk budget constraints would find optimality. Within the context of insurer capital from an S\&P Rating perspective we manage the portfolio within certain constraints. Generally speaking we charge Public Equity a 45\% capital charge and Private Equity a 54\% capital charge. I have attached the S\&P Capital methodology in case you want to dive deeper. In the context of our portfolio I think a reasonable assumption could be to set the risk budget constraint between 25\%-35\% thus implying an allocation between 50\% to 70\% to equity.
        \item $\lambda_{N}$: Historically has been observed that capital calls go below historical averages during an economic downturn as deal flow generally stops during these periods. That is already reflected in the numbers you have for $\lambda_{K}$ which make sense to me. For $\lambda_{N}$, I think both $s=1$ and $s=2$ need to be revised. I have looked at our PE Buyout portfolio data on a deal by deal basis. The chart below shows the \% of capital contribution within the quarter when the commitment was closed and the end of subsequent quarter. For $\lambda_{N}$, after adjusting for the timing of when the commitment closing might have actually take place during the quarter, I would suggest using a $\lambda_{N}$ of 0.039. I would also suggest keeping this number the same for $s=1$ and $s=0$ as it is subject more to idiosyncratic factors.
    \end{itemize}
    \item Citations:
        \begin{itemize}
          \item Work in \citet{boyd/etal:22}.
        \end{itemize}
\end{enumerate}

\clearpage 
